Reasoning Over Virtual Knowledge Bases With Open Predicate Relations

We present the Open Predicate Query Language (OPQL); a method for constructing a virtual KB (VKB) trained entirely from text. Large Knowledge Bases (KBs) are indispensable for a wide-range of industry applications such as question answering and recommendation. Typically, KBs encode world knowledge in a structured, readily accessible form derived from laborious human annotation efforts. Unfortunately, while they are extremely high precision, KBs are inevitably highly incomplete and automated methods for enriching them are far too inaccurate. Instead, OPQL constructs a VKB by encoding and indexing a set of relation mentions in a way that naturally enables reasoning and can be trained without any structured supervision. We demonstrate that OPQL outperforms prior VKB methods on two different KB reasoning tasks and, additionally, can be used as an external memory integrated into a language model (OPQL-LM) leading to improvements on two open-domain question answering tasks.

==> results.tex <==
\section{Experiments \label{sec:results}}
We experimented \tae{} on two sets of experiments: multi-hop relational following over a virtual KB, and injecting \tae{} memory into a language model to improve the performance of open-domain QA.
% Experiments:
% \begin{enumerate}
% \item KB completion
% \item Zero shot relation prediction
% \item Structural relations on KB without a KB
% \item Multihop (complex webQ)
% \item Dr Kit comparisons
% \end{enumerate}

\noindent\textbf{Pretraining Data: }
% \tae{} is pretrained on entity-linked documents. In our experiments, 
We use Wikipedia passages with hyperlinks as our pretraining. The hyperlinks link a span of tokens to a Wikipedia page for an entity $e$. The spans of tokens that are linked are considered as mentions, and entity $e$ is the corresponding entity.
%Entities in Wikipedia  and utilize the hyperlinks in the text as entity linking. 
We take the 1M most frequent entities in Wikipedia as our entity vocabulary $\mathcal{E}$. Passages are split into text pieces with every 128 tokens. We count the pairs of entities that co-occur in the same text pieces, and filtered the pairs by their frequency and point-wise mutual information (PMI). The top 800k pairs of entities are selected as our candidates for training. During training, an input with pair $(e_1, e_2)$ will be paired with $2$ positive examples that mentions the same pair of entities, and $8$ hard negative examples $(e_i, e_j)$ that mention either the same topic or target entities, i.e. $e_i = e_1$ or $e_j = e_2$, but not both. Batch negatives are also included in pretraining. 















% \section{Experiments \label{sec:results}}
% We experimented \tae{} on two sets of experiments: multi-hop relational following over a virtual KB, and injecting \tae{} memory into a language model to improve the performance of open-domain QA.
% % Experiments:
% % \begin{enumerate}
% % \item KB completion
% % \item Zero shot relation prediction
% % \item Structural relations on KB without a KB
% % \item Multihop (complex webQ)
% % \item Dr Kit comparisons
% % \end{enumerate}

% \noindent\textbf{Pretraining Data: }
% % \tae{} is pretrained on entity-linked documents. In our experiments, 
% We use Wikipedia passages with hyperlinks as our pretraining. The hyperlinks link a span of tokens to a Wikipedia page for an entity $e$. The spans of tokens that are linked are considered as mentions, and entity $e$ is the corresponding entity.
% %Entities in Wikipedia  and utilize the hyperlinks in the text as entity linking. 
% We take the 1M most frequent entities in Wikipedia as our entity vocabulary $\mathcal{E}$. Passages are split into text pieces with every 128 tokens. We count the pairs of entities that co-occur in the same text pieces, and filtered the pairs by their frequency and point-wise mutual information (PMI). The top 800k pairs of entities are selected as our candidates for training. During training, an input with pair $(e_1, e_2)$ will be paired with $2$ positive examples that mentions the same pair of entities, and $8$ hard negative examples $(e_i, e_j)$ that mention either the same topic or target entities, i.e. $e_i = e_1$ or $e_j = e_2$, but not both. Batch negatives are also included in pretraining. 





% \subsection{Reasoning Over VKB \label{sec:exp_reasoning}}
% \subsubsection{Datasets}
% We evaluated \tae{} on two semi-structured multi-hop QA datasets. \hs{Add dataset stats.}

% \textbf{MetaQA} \hs{cite} is a multi-hop QA dataset that extends the WikiMovies dataset to 2-hop and 3-hop questions in the movie domain. The questions are generated from templates, e.g. "Who starred in the movies directed by Christopher Nolan". Questions in MetaQA are answerable by the corpus provided in the original WikiMovies dataset. The corpus contains 18k passages that describes the relations between 43k entities. We extracted 106k entity pairs from the corpus whose topic entity is the Wikipedia page title and target entity is one of the mentions in the passage. Reverse pairs are also included, making a total of 213k entity pairs in the vocabulary.

% \textbf{Multi-hop Slot Filling (MSF)} \hs{cite} is a large scale multi-hop reasoning dataset constructed on WikiData that contains 120k passages, 888 relations, and more than 200k entities. Queries are constructed from multi-hop paths from WikiData and turned in into natural language questions concatenating the head entity with the path of relations, e.g. (``Steve Jobs'', founder, headquarter in, ?). Similar to MetaQA, we constructed entity pairs by taking the Wikipedia page title as the topic entity and entities mentioned in the passages as target entities. We extracted 1.3m and 781k entity pairs for 2-hop and 3-hop questions.

% \subsubsection{Baselines}
% GRAFT-Net \cite{sun2018open} is a Graph-CNN based model that can perform reasoning jointly over text and knowledge bases. PullNet \cite{sun2019pullnet} extends GRAFT-NET by introducing an iterative retrieve-and-classify mechanism to solve complex questions. PIQA \cite{seo-etal-2018-phrase} and DrKIT \cite{dhingra2019differentiable} built mention-level index using a pretrained encoder. A retriever model is learned to retrieve from the pretrained index to answer open-domain questions. Pretraining the DrKIT index requires distant supervision using artificial queries constructed from the KB. KV-Mem \cite{miller2016key} are DrQA \cite{chen2017reading} are another two famous open-domain QA baselines.

% \subsubsection{Results}
% % We first build the \tae{} memory using the pretrained relation encoder. The MetaQA corpus contains information about movies, such as directors, actors, and genre, etc. We take the name of a movie as the topic entity, and all other information as target entities, e.g. $(\textit{Inception}, \textit{Christopher Nolan})$. We also include inverse pairs $(\textit{Christopher Nolan}, \textit{Inception})$. 

% We experiment on the relational following task using both a pretrained memory (\tae{}-pretrained) and a finetuned memory (\tae{}). We evaluated the Hits@1 performance of the model. The results are listed in Table \ref{tab:reasoning}. The pretrained memory is directly built using the pretrained relation encoder from common Wikipedia pairs. 
% Without any finetuning of the relation encoder, 
% \tae{} with pretrained memory achieves the state-of-the-art performance on both MSF 2-hop and 3-hop datasets. \tae{}-pretrained is slightly lower than DrKIT on the MetaQA, because DrKIT finetuned its mention encoder on the MetaQA corpus. The MetaQA corpus only contains 14 relations (including their inverse) in the movie domain, so it's easy for the model to learn only capturing these relationship between entities. To resolve this bias, we finetune the \tae{} relation encoder on the MetaQA corpus. The finetuning data is distantly constructed from 1-hop questions in the MetaQA dataset, by masking the topic entity from the question and inserting a placeholder for the target entity at the end of the question. We end up with 10K finetuning data for the relation encoder for MetaQA. Similarly, we constructed 19K finetuning data for the MSF dataset. The performance of \tae{} with the finetuned memory outperforms DrKIT on 2-hop questions by 2.5 points and becomes very comparable on 3-hop questions.

% \begin{table}[h]
%     \small
%     \centering
% \begin{tabular}{l|cc|cc}
%  \toprule
%   & \multicolumn{2}{c}{MetaQA} & \multicolumn{2}{|c}{MSF} \\
%   Model & 2Hop & 3Hop & 2Hop & 3Hop \\
%   \midrule 
%   KVMem  & 7.0 & 19.5 & 3.4  & 2.6 \\
%   DrQA  & 32.5 & 19.7 & 14.1 & 7.0 \\
%   GRAFT-Net  & 36.2 & 40.2 & -  & - \\
%   PullNet  & 81.0 & 78.2 &  - & - \\
%   PIQA  & -  & - & 36.9 & 18.2  \\
%   DrKIT & 86.0 & \textbf{87.6}  & 46.9 & 24.4 \\
%   \midrule
%   \tae{} & \textbf{88.5} & 87.1  & \textbf{49.2} & \textbf{29.7}  \\
%     ~~ - finetune rel  & 84.7 & 84.3  &48.5 & 28.1\\
% \bottomrule
% \end{tabular}
%     \caption{\textbf{Multi-hop relational following}. (+finetune rel) finetune the relation encoder. \hs{describe eval metrics.} \label{tab:reasoning}}
% \end{table}

% % \begin{table}[h]
% %     \small
% %     \centering
% % \begin{tabular}{l|cc}
% %  \toprule
% %   & \multicolumn{2}{c}{MSF} \\
% %   Model & 2Hop & 3Hop \\
% %   \midrule
% %   \tae{} & \textbf{48.5} & \textbf{28.1} \\
% %   \midrule
% %   DrQA(ots, cascade)  & 14.1 & 7.0  \\
% %   PIQA (ots, cascade)  & 11.8 & 6.4 \\
% %   \midrule 
% %   PIQA (pre, cascade)  & 36.9 & 18.2 \\
% %   DrKIT (pre, cascade)  & 40.4 & 19.8 \\
% %   DrKIT (e2e)  & 46.9 & 24.4 \\
% % \bottomrule
% % \end{tabular}
% %     \caption{\textbf{}.  \label{tab:reasoning}}
% % \end{table}

% \subsubsection{Generalize to Novel Relations}
% One benefit of the \tae{} is that the pretraining process does not require any signal from knowledge bases, so the capacity of \tae{} memory is ideally unlimited. On the contrary, while training DrKIT requires distantly supervision from knowledge base, this restrict the capacity of DrKIT to only encode KB relations seen at pretraining time. To demonstrate this difference, we hold out some portions of relations in the pretraining phase of DrKIT but evaluate on queries that at least one of the held-out relations is required to answer the queries. We compare DrKIT to the pretrained \tae{} memory. The result is shown in Table \ref{tab: abl-holdout-rel}. \hs{compare results.}

% We show that the pretrained \tae{} relation encoder can effective

% \begin{table}[h]
%     \small
%     \centering
% \begin{tabular}{l|ccc|ccc}
%  \toprule
%   & \multicolumn{3}{c}{MSF-2hop} & \multicolumn{3}{|c}{MSF-3hop} \\
%   Model & 10\% & 20\% & 50\% & 10\% & 20\% & 50\% \\
%   \midrule
%   \# data & 1746 & 4514 & 7848 & 2524 & 5628 & 9100 \\
%   \midrule
%   DrKIT & & & & & & \\
%   \tae{} & 48.6 & 51.8 & 49.0 & 31.7 & 28.4 & 27.6 \\
% \bottomrule
% \end{tabular}
%     \caption{Evaluation with \% of heldout relations. \hs{turn this into figures.} \label{tab: abl-holdout-rel}}
% \end{table}




% \subsection{Injecting VKB into Language Models \label{sec:exp_lm}}

% % \pat{Discuss memory updating connections to FaE and dataset specific results. Our model allows us to update the memory without retraining for optimizing a specific application.}
% \subsubsection{Dataset}
% \textbf{WebQuestionSP} (WebQSP) \hs{cite} is an open-domain Question Answering dataset that contains 4737 factual questions. The questions are answerable using entities in Freebase. 

% \textbf{ComplexWebQuestions} (ComplexWebQ) \hs{cite} is a multi-hop entity-based question answering dataset that contains 34,689 complex questions, including 45\% composition questions, 45\% conjunction questions, and 10\% others.

% \subsubsection{Baselines}
% \hs{Add citations} We compare \tae{} with several strong open-domain QA baselines. GRAFT-Net is a Graph-CNN based model that can perform reasoning jointly over text and knowledge bases. PullNet extends GRAFT-NET by introducing an iterative retrieve-and-classify mechanism to solve complex questions. BART and T5 are large pretrained text-to-text Transformer models. EaE learns contextual representations for entities from text is trained to retrieve the entities from an external memory. Different from \tae{}, EaE does not have an external reasoning modele, so it requires the reasoning process performed all inside the Language Model. DPR is a retrieve-and-read approach that pairs a dense retriever in the embedding space with a BERT based reader. To extend DPR to handle multi-hop questions, we concatenate answers from the previous hops to the question as the query for the next hop. This is referred as DPR-cascade.

% \begin{table}[h]
%     \small
%     \centering
% \begin{tabular}{l|ccc}
%  \toprule
%   Model & WebQSP & ComplexWebQ (dev) \\
%   \midrule
% %   tfidf NN & 21.4  & - \\
% %   Dense NN & 27.8  & - \\
%   GRAFT-NET  & 25.3  & 10.6 \\
%   PullNet  & 24.8 & 13.1 \\
%   BART-Large  & 30.4  & - \\
%   EaE  & 47.4  & 31.3 \\
%   T5  & 49.7  & 38.7 \\
%   DPR  & 48.6  & 24.6 \\
%   DPR-cascade & - & 25.1 \\
%   \midrule
%   \tae{}-follow & 46.6 & 18.5 \\
%   \tae{}-LM  & \textbf{51.9} & \textbf{40.9}\\
% %   ~~ + webqsp mem & 53.7  & -\\
%   \midrule
%   \midrule
%   FaE  & 54.7 & -\\
%   SplitQA & -  & 29.0 \\
%   NSM  & 69.0 (F1) & \\
%   PullNet (KB) & - & 47.2 \\
  
% \bottomrule
% \end{tabular}
%     \caption{\tae{}-follow directly takes the retrieval results as answers. \tae{}-LM mixed the embeddings with language model and then make predictions. (+webqsp mem) swaps in the dataset specific memory, while \tae{}-follow and \tae{}-LM use the same memory from pretraining. T5-11B for WebQSP. T5-3B for ComplexWebQ. \label{tab:reasoning}}
% \end{table}


% \begin{table}[h]
%     \small
%     \centering
% \begin{tabular}{l|ccc}
%  \toprule
%   Model & WebQSP & ComplexWebQ (dev) \\
%   \midrule
%   \tae{}-LM  & 51.9 & 40.9\\
%   ~~ + webqsp mem & 53.7  & 41.1\\
% \bottomrule
% \end{tabular}
%     \caption{Injecting new entries to memory. \label{tab:reasoning}}
% \end{table}


% % %%% WQSP
% % \begin{table*}[t]
% %     \small
% %     \centering
% % \begin{tabular}{ll|cc|cc|cc|cc}
% %  \toprule
% %  & &  \multicolumn{4}{c|}{WebQuestionsSP} & \multicolumn{4}{c}{TriviaQA} \\
% %     & Model      &   \multicolumn{2}{c|}{Full Dataset} & \multicolumn{2}{c|}{Wikidata Answer}   &  \multicolumn{2}{c|}{Full Dataset} &                \multicolumn{2}{c}{Wikidata Answer}  \\
% %  &           & Total      & No Overlap &  Total      & No Overlap  & Total      & No Overlap &  Total      & No Overlap \\
% % \toprule
% % \multirow{1}{*}{\textit{Ours}} & \tae{} FILM & -      & - & -  & -  & -  & - & - & - \\
% % \midrule
% % \multirow{6}{*}{\textit{Closed-book}} 
% % & FaE & {54.7}           & {36.4} & {78.1}  & {72.2} 
% %     & {29.1}           & {15.6} & {37.3} & {28.4} \\
% % & EaE             & 47.4          & 25.1  & 62.4 & 42.9  
% %     & 19.0          & 9.1 & 24.4  & 17.1 \\
% % % \bottomrule
% % &T5-11B              & 49.7          & 31.8     & 61.0  & 48.5    
% %     &  --           & -- &  --  & -- \\
% % &BART-Large            & 30.4          & 5.6  & 36.7  & 8.3    
% %     & 26.7          & 0.8  & 30.6 & 1.0 \\
% % &Dense NN        & 27.8            & 2.9 & 34.0  & 3.8  
% %     & 28.9            & 0.0 & 33.2 & 0.0 \\ 
% % &tfidf NN        & 21.4         & 2.6 & 25.4  & 3.0    
% %     & 23.5           & 0.0 & 26.9 & 0.0 \\
% % \midrule    
% % \multirow{ 3}{*}{\textit{Open-Book}}
% % &RAG             & {50.1}          & {30.7} & {62.5}  & {45.1}    
% %     & 56.8          & 29.2 & 64.9  & 45.2\\
% % &DPR             & 48.6         & 34.1 & 56.9 & 45.1 
% %     & 57.9         & 31.6 & 66.3 & 48.8 \\
% % &FID             &  --           & -- &  --  & --   
% %     &  {67.6}           & {42.8} &  {76.5}  & {64.5} \\
% % % \midrule
% % % &EmQL\dag           &  \textbf{75.5}  & - &  74.6 & - & - & - & - & - \\
% % \bottomrule
% % \end{tabular}
% %     \caption{\textbf{Open Domain QA Results}. Columns denoted \textit{Full Dataset-Total} are conventional splits discussed in \S \ref{sec:main_results}, \textit{Wikidata Answer} are answerable using Wikidata (\S \ref{sec:wikidata_answerable}), and \textit{No Overlap} removes train-test overlap (\S \ref{sec:data_overlap}).  Other than \tae{}\_\mac{}, \mac{}, and EaE, all results are derived from the prediction files used in \citet{lewis2020question} including the nearest neighbor (NN) baselines. \label{tab:lmqa}}
% % \end{table*}


% % \subsubsection{WebQuestionsSP}

